Generalized Relative Neighborhood Graph (GRNG) for Similarity Search

Similarity search is a fundamental building block for information retrieval on a variety of datasets. The notion of a neighbor is often based on binary considerations, such as the k nearest neighbors. However, considering that data is often organized as a manifold with low intrinsic dimension, the notion of a neighbor must recognize higher-order relationship, to capture neighbors in all directions. Proximity graphs, such as the Relative Neighbor Graphs (RNG), use trinary relationships which capture the notion of direction and have been successfully used in a number of applications. However, the current algorithms for computing the RNG, despite widespread use, are approximate and not scalable. This paper proposes a novel type of graph, the Generalized Relative Neighborhood Graph (GRNG) for use in a pivot layer that then guides the efficient and exact construction of the RNG of a set of exemplars. It also shows how to extend this to a multi-layer hierarchy which significantly improves over the state-of-the-art methods which can only construct an approximate RNG.

==> assets/figures/2L_GRNG_RNG_Results/fig_supplementary_GRNG_RNG_Fixed_N_Results.tex <==
\begin{figure}[h!]
    \centering
    % %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    % (or a blank line to force the subfigure onto a new line)
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_stage_search_distances.pdf}
    \end{minipage}
    %
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_stage_index_distances.pdf}
    \end{minipage}
    
    
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_stage_search_time.pdf}
    \end{minipage}
    %
    \begin{minipage}{0.45\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_stage_index_time.pdf}
    \end{minipage}
    
    \begin{minipage}{0.31\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_radii.pdf}
    \end{minipage}
    %
    \begin{minipage}{0.31\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_memory.pdf}
    \end{minipage}
    %
    \begin{minipage}{0.31\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/2L_GRNG_RNG_Results/Opt_FixedN_GRNG_RNG_degree.pdf}
    \end{minipage}
    
    \caption{\footnotesize Statistics for the optimization of a 2-Layer GRNG-RNG hierarchy with a fixed $N=102,400$ on 2D, uniformly distributed data.}
    \label{fig:supplementary_GRNG_RNG_Fixed_N_Results}
\end{figure}


==> assets/proofs/proof_prop7.tex <==
%% PROOF TO PROP 7
\begin{proof}
    Apply Theorem~\ref{thm:GRNG_S1} with $(\bar{p}_{\bar{j}},\bar{r}_{\bar{j}})$ acting both as a coarse-scale pivot $(p_j,r_j)=(\bar{p}_{\bar{j}},\bar{r}_{\bar{j}})$ and as a fine-scale pivot. Thus, constituents of $(p_i,r_i)$, say $(Q,\bar{r}_Q)$, cannot form a GRNG link with constituents of $(p_j,r_j)$, \textit{i.e.,} the sole constituent, $(\bar{p}_{\bar{j}},\bar{r}_{\bar{j}})$.
    \qed
\end{proof}

==> assets/tables/results_real/results_COREL.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Algorithm} & \textbf{Total Links} & \textbf{Extra (+) and Missing (-) Links} & \textbf{Average Degree}        & \textbf{Search Distances} & \textbf{Index Construction Distances} \\ \hline \hline
Hacid et. al       & 212,211              & 21,802/-4                                & 6.2378                         & 177,972.36                & 9,823,840,198,726                     \\ \hline
Rayar et. al       & 190,908              & 535/-40                                  & 5.6116 & 169,575.08                & 6,432,673,175                         \\ \hline
Ours               & 190,413              & 0/-0                                     & 5.5971 & 43,729.20                 & 1,611,369,217                         \\ \hline
\end{tabular}

==> assets/tables/results_real/results_LA.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Algorithm}    & \textbf{Total Links} & \textbf{Extra (+) and Missing (-) Links} & \textbf{Average Degree}                 & \textbf{Search Distances} & \textbf{Index Construction Distances} \\ \hline \hline
Hacid et. al & \multicolumn{5}{c|}{Impractical}           \\ \hline

Rayar et. al & 1,277,369   & +3,254/-33,706* & 2.3793  &   2,147,498.42   & 1,153,035,099,784                     \\ \hline
Ours         & 1,307,821   & -               & 2.4360  &   1,020.71       & 1,042,175,220                         \\ \hline

\end{tabular}

==> assets/tables/results_real/results_MNIST.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Algorithm} & \textbf{Total Links} & \textbf{Extra (+) and Missing (-) Links} & \textbf{Average Degree}        & \textbf{Search Distances} & \textbf{Index Construction Distances} \\ \hline \hline
Hacid et. al       & 118,248              & +3,778/-3                                & 3.9416                         & 87,713.10                 & 1,430,022,984,523                     \\ \hline
Rayar et. al       & 114,893              & +865/-445                                & 3.8298 & 88,172.04                 & 2,639,416,420                         \\ \hline
Ours               & 114,473              & +0/-0                                    & 3.8158 & 10,058.90                 & 407,689,553                           \\ \hline
\end{tabular}
